Multi-armed Bandit and Backbone boost Lin-Kernighan-Helsgaun Algorithm for the Traveling Salesman Problems

The Lin-Kernighan-Helsguan (LKH) heuristic is a classic local search algorithm for the Traveling Salesman Problem (TSP). LKH introduces an $\alpha$-value to replace the traditional distance metric for evaluating the edge quality, which leads to a significant improvement. However, we observe that the $\alpha$-value does not make full use of the historical information during the search, and single guiding information often makes LKH hard to escape from some local optima. To address the above issues, we propose a novel way to extract backbone information during the TSP local search process, which is dynamic and can be updated once a local optimal solution is found. We further propose to combine backbone information, $\alpha$-value, and distance to evaluate the edge quality so as to guide the search. Moreover, we abstract their different combinations to arms in a multi-armed bandit (MAB) and use an MAB model to help the algorithm select an appropriate evaluation metric dynamically. Both the backbone information and MAB can provide diverse guiding information and learn from the search history to suggest the best metric. We apply our methods to LKH and LKH-3, which is an extension version of LKH that can be used to solve about 40 variant problems of TSP and Vehicle Routing Problem (VRP). Extensive experiments show the excellent performance and generalization capability of our proposed method, significantly improving LKH for TSP and LKH-3 for two representative TSP and VRP variants, the Colored TSP (CTSP) and Capacitated VRP with Time Windows (CVRPTW).

==> 04-Recollect.tex <==
% 在这部分为介绍将要提出的算法做一些前驱工作。本节将要介绍1-tree和k-opt算法，和基于这些算法之上的优秀的LKH算法。
In this section, some preliminary work will be done to introduce the \name algorithm. This section will introduce several important parts which consists of 1-tree' $\alpha$-value, penalties, candidates and k-opt operation in LKH algorithms~\cite{Helsgaun2000,Helsgaun2009}.% (described in Section \ref{sec-usage}).

%\subsection{Definitions of the Problems and Concepts}
\subsection{$\alpha$-value Calculated by 1-tree and Candidates}
\label{sec-def}
% % 经过多年来大师们的改良，LK算法已经是集大成之作。而LKH算法更是经典中的经典，虽然距离算法的提出已经过去多年，但是仍有众多的研究者慕名而来。同时LKH也被工业化集成，源码可以在官网上找见。
% After years of improvement by masters, the LK algorithm has become a masterpiece. The LKH algorithm is even more classic among the classics. Although the distance algorithm has been proposed for many years, many researchers still come to admire it. At the same time, LKH has also been industrialized and integrated, and the source code can be found on the official website. 


% 1-tree是最小生成树的一种变体。在n个结点1,2,...,n中,1-tree 是由结点2,3,...n 组成的树，并且和顶点1有两条边相邻接。如果1-tree中的每个点的度数均为2，则其构成了一条旅行回路。给定图G=(V,E)，其中V是点的结合，E是边的集合,(i,j)表示图中i和j之间的边，(i,j)∈E,且i,j∈V。V是由结点1,2,...,n的结点构成的点集。定义L(T)为图G中最小1-tree花费的代价，L(T(i,j))是包含(i,j)这条边所构成的最小1-tree的代价。定义\ensuremath{\alpha}的计算公式如下
1-tree is a variant of Minimum Spanning Tree(MST). We have n nodes numbered by 1, 2, ... , n respectively. 1-tree is composed of nodes 2, 3, ... , n, and adjacent to vertex 1 with two edges. If each point in the 1-tree has a degree of 2, it constitutes a travel loop. In a symmetric graph $G= (V, E)$, $V$ is a set of points, $E$ is a set of edges and $(i, j)$ represents the edges between $i$ and $j$ in the graph. $E$ is composed of $(i, j)$. $V$ is composed of vertices 1, 2, ... , i, j, ... , n. Define $L(T)$ as the cost of the smallest 1-tree in Figure $G$, and $L(T(i, j))$ is the cost of the smallest 1-tree contains the edge $(i, j)$. Define $\alpha(i, j)$ is a value measuring the quality of edge $(i,j)$. The calculation formula for \ensuremath{\alpha(i, j)} is as follows. 

\begin{equation}
\label{eq_alpha}
\ensuremath{\alpha(i,j)} = L(T(i,j)) - L(T)
\end{equation}

% LKH是在利用1-tree计算出α值，在此基础上之上利用k-opt算法进行局部搜索，得到了优秀的实验结果。值得一提的是，α值是选择一条边时候的重要参考，α的值越小，代表这条边越有可能是局部最优中的一部分。
Equation \ref{eq_alpha} means the gap between MST has the edge (i,j) and $L(T)$.
Therefore, the \ensuremath{\alpha} value is an important reference when selecting an edge. The smaller the value of, the more likely this edge is to be a part of the local optimum.

% 通过1-tree计算得到的α可以定义每个结点侯选边的优先级。LKH中选择侯选边依赖于定义好的优先级。好的侯选边可以帮助算法更快找到更低的山谷，加快算法的收敛。！！！文章实验证明α对于侯选边的设置对启发式算法的局部搜索起到了关键的作用。LKH算法会优先选择α值小的侯选边进行k-opt操作，同时会动态调整结点候选边集合，贪心地加入当前最好的边，同时删除不可能或者重复的边，以此来优化算法的寻优过程。
Define the priority of each node's candidate edges using $\alpha(i, j)$ called $\alpha$-value for convenience in the following. The selection of candidate edges in LKH depends on the defined priority of edge. Good candidate edges can help the algorithm find better local optima faster and accelerate the convergence of the algorithm. Experimental in LKH proofs $\alpha$-value the setting of candidate edges plays a crucial role in the local search of heuristic algorithms. LKH algorithm will execute k-opt operation prioritizing the edge candidate with smaller $\alpha$-value, while dynamically adjusting the set of node candidate edges with greedily adding the edge in current best solution and deleting impossible or repetitive edges to optimize the algorithm's process in searching~\cite{Helsgaun2000}.


\subsection{Penalties for Maximum Lower Bound}

In this part, we will introduce the penalty used to calculate maximum lower bound for instance, which is an important property for LKH worth mentioning. Assuming that each node has a corresponding penalty. $\pi$ is composed of $\pi_1$,$\pi_2$,...,$\pi_n$. These penalties are also adjusted by a Based on these penalties, the distance of each node can be reconstructed by \ref{penalty}.
\begin{equation}
\label{penalty}
C(i,j) = d(i,j) + \pi_i + \pi_j         
\end{equation}
$d(i, j)$ is the distance between node i and node j. $C(i, j)$ is the distance decorated by $\pi_i$ and $\pi_j$. If we replace $d(i, j)$ with $C(i, j)$, the result of TSP is invariant but it will change the minimum 1-tree.
Besides, LKH uses this method to maximize the lower bound of the optimal TSP solution by adding penalties. Define $L(T(\pi))$ is the length of the minimum 1-tree after adding the penalties. the lower bound $\omega(\pi)$ can be caculated by the formulation.
\begin{equation}
\omega(\pi) = L(T(\pi)) - 2\sum_i \pi_i
\end{equation}
LKH algorithm maximums the lower bound of $\omega(\pi)$ while chaning $\pi$. In addition, the better lower bound is found, the better $\alpha$-value will be set and the smaller $\alpha$-value is, the higher quality candidate edge has. At last, every city will determine candidate edges using five smallest $\alpha$-value which are an essential part of k-opt operation for reconstruct hamilton curcuit.

\subsection{k-opt Operation in LKH}
\label{sec-single}

Local search with k-exchange neighborhoods, k-opt, is the most widely used heuristic method for the TSP. Before starting the algorithm \ref{alg_single}, some symbolic explanations need to be made. $P_i$ represents city and index $i$ means its serial number. In addition, $(P_{2i-1}, P_{2i-1})$ exists in current tour T, while $(P_{2i}, P_{2i+1})$ is the edge that possible to add in the T. In k-opt algorithm, there are two key constraints C1 and C2. We define the two constraints are called feasible rule and positive rule respectively.

\begin{itemize}
\item C1: After $k$ times search, connecting $P_{2k}$ to $P_1$ should generate a feasible TSP tour.
\item C2: Gain should be positive which means $\sum_{i=1}^k(d(P_{2i-1}, P_{2i})-d(P_{2i}, P_{2i+1})) > 0$.
\end{itemize}


\begin{algorithm}[t]
\NoCaptionOfAlgo
\caption{Algorithm 1. k-opt in LKH}
\label{alg_single}
\LinesNumbered
\KwIn{old tour: $x_{in}$, $G(V,E)$, current search depth: $k$, maximum search depth: $k_{max}$, the starting city: $P_1$, sequence of corresponding cities: $P$}
\KwOut{new tour: $x_{out}$, sequence of the corresponding cities: $P$}
\For{$i = 1 : 2$}{
    $P_{2k} \leftarrow P_{2k-1}^{i}$;

    \If{$P_{2k}$ does not obey feasible rule $C1$}{
        \textbf{continue}};
    \If{$k >= 2 \land \sum_{j=1}^{k}d(P_{2j-1}, P_{2j}) < \sum_{j=1}^{k-1}d(P_{2j}, P_{2j+1}) + d(P_{2k},P_{1} $)}{
        $x_{out} \leftarrow x_{in}$;
        
        \For{$j = 1:k$}{
            remove edge $(P_{2j-1}, P_{2j})$ from $x_{out}$;
        }
        \For{$j = 1:k-1$}{
            add edge $(P_{2j}, P_{2j+1})$ into $x_{out}$;
        }
        add edge $(P_{2k}, P_{1})$ into $x_{out}$;
        
        \textbf{return} $(x_{out}, P)$;
    }
    \If{$k = k_{max}$}{\textbf{return} $(x_{in},\emptyset)$;}
    \For{$j = 1:5$}{
        $P_{2k+1}$ = the $j$-th  city in $P_{2k}$'s candidate set;
        
        \If{$P_{2k+1}$ does not obey the gain constraint $C2$}{\textbf{continue};}
        $(x_{temp}, P^{'}) \leftarrow k-opt(x_{in}, G(V,E), P_{1}, P \cup (P_{2k}, P_{2k+1}), k+1, k_{max});$
        
        \If{$l(x_{temp}) < l(x_{in})$}{\textbf{return} $(x_{temp}, P^{'})$;}
    }
}
\textbf{return} $(x_{in}, \emptyset);$
\end{algorithm}

In the algorithm 1, programe input tour $x_{in}$, $G$ consisting of $V$ and $E$, current searching depth $k$, maximum searching depth, starting city $P_1$ and sequence of corresponding cities $P$. The program finally output new tour $x_{out}$ and sequence of corresponding cities $P$. The algorithm starts from $P_1$ choosing its successor or precursor(line 1-2). It checks feasible rule before the algotirhm starts(line 3- 4). If improvement is found, update $x_{out}$ with adding and removing related edges(line 5- 11). Whats' more, the algorithm allows that explored edges can be search once again. Line 12 means once a improvement is found and then return the current new result. The algorithm will also end when search depth reaches $k_{max}$ depth(line 13, 14). Moreover, the default candidate set size for each node is 5. Therefore, index $j$ ranges from 1 to 5 and the algorithm does recursive operation during the research(in line 15- 22).


After introducing k-opt algorithm which is a main part of LKH algorithm, main body of LKH will be represented well appearing in the \name in the next session.

==> table-Main.tex <==
\begin{table*}[!t]
\caption{Detailed comparison results of \name and LKH on all 45 tested instances. The best results appear in \bf{bold}.}
\centering
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{lr:rrrrrrrrrr} \toprule
\multirow{2}{*}{Instance} & \multirow{2}{*}{Optimum} & \multicolumn{54}{c:}{LKH}                                                                        & \multicolumn{54}{c}{MABB-LKH\name}                                         \\ \cline{3-12} 
                          & &                       & Success & Best                          & Average                         & Trials  & Time(s)  & Success & Best            & Average             & Trials  & Time(s)  \\ \hline
\multicolumn{2}{l:}{\textit{Easy}   instances}              &         &                               &                                 &         &          &         &                 &                     &         &          \\
att532                    & 27686                 & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 71.2    & 0.42     & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 72.3    & 0.40     \\
ali535                    & 202339                & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 4.9     & 0.12     & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 4.9     & 0.12     \\
pa561                     & 2763                  & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 58.5    & 0.49     & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 41.1    & 0.39     \\
u574                      & 36905                 & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 149.9   & 0.97     & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 51.1    & 0.41     \\
p654                      & 34643                 & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 22.9    & 7.78     & 10/10& 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 22.9    & 7.86     \\
d657                      & 48912                 & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 46.2    & 0.28     & 10/10& 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 47.0    & 0.25     \\
u724                      & 41910                 & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 125.4   & 1.78     & 10/10& 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 119.0   & 1.57     \\
rat783                    & 8806                  & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 4.2     & 0.11     & 10/10& 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 4.2     & 0.10     \\
dsj1000                   & 18660188              & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 366.8   & 6.74     & 10/10& 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 245.9   & 5.92     \\
si1032                    & 92650                 & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 152.0   & 22.71    & 10/10& 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 67.1    & 10.54    \\
u1432                     & 152970                & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 5.3     & 0.65     & 10/10& 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 5.3     & 0.64     \\
d1655                     & 62128                 & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 194.1   & 2.18     & 10/10& 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 121.2   & 1.98     \\
u2319                     & 234256                & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 3.1     & 1.09     & 10/10& 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 3.1     & 1.02     \\
pr2392                    & 378032                & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 5.8     & 1.00     & 10/10& 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 24.2    & 10.10    \\
pla7397                   & 23260728              & 10/10  & \textbf{Opt.}                 & \textbf{Opt.}                   & 632.4   & 198.39   & 10/10& 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 224.7   & 174.15   \\ \hline
\multicolumn{2}{l:}{\textit{Hard}   instances}              &         & \textbf{}                     & \textbf{}                       &         &          &         & \textbf{}       & \textbf{}           &         &          \\
si535                     & 48450                 & 7/10   & \textbf{Opt.}                 & 48451.1                         & 311.6   & 21.28    & 8/10& 8/10   & \textbf{Opt.}   & \textbf{48450.8}    & 290.3   & 15.52    \\
rat575                    & 6773                  & 2/10   & \textbf{Opt.}                 & 6773.8                          & 526.9   & 2.32     & 4/10& 4/10   & \textbf{Opt.}   & \textbf{6773.6}     & 446.7   & 2.49     \\
gr666                     & 294358                & 5/10   & \textbf{Opt.}                 & \textbf{294417.0}               & 459.8   & 2.41     & 2/10& 2/10   & \textbf{Opt.}   & 294452.4            & 567.8   & 2.89     \\
pr1002                    & 259045                & 8/10   & \textbf{Opt.}                 & 259045.6                        & 549.0   & 3.13     & 10/10& 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 172.8   & 1.10     \\
u1060                     & 224094                & 5/10   & \textbf{Opt.}                 & 224107.5                        & 663.3   & 84.17    & 9/10 & 9/10   & \textbf{Opt.}   & \textbf{224096.7}   & 182.7   & 30.02    \\
vm1084                    & 239297                & 3/10   & \textbf{Opt.}                 & 239372.6                        & 824.1   & 32.98    & 5/10   & \textbf{Opt.}   & \textbf{239336.0}   & 767.0   & 35.48    \\
pcb1173                   & 56892                 & 4/10   & \textbf{Opt.}                 & 56895.0                         & 844.0   & 3.92     & 6/10   & \textbf{Opt.}   & \textbf{56894.0}    & 658.2   & 4.11     \\
d1291                     & 50801                 & 5/10   & \textbf{Opt.}                 & 50840.0                         & 995.4   & 27.44    & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 614.1   & 15.18    \\
rl1304                    & 252948                & 3/10   & \textbf{Opt.}                 & 253156.4                        & 1170.0  & 12.48    & 7/10   & \textbf{Opt.}   & \textbf{252996.4}   & 663.4   & 12.21    \\
rl1323                    & 270199                & 6/10   & \textbf{Opt.}                 & 270219.6                        & 718.8   & 9.63     & 8/10   & \textbf{Opt.}   & \textbf{270204.4}   & 641.7   & 8.51     \\
nrw1379                   & 56638                 & 6/10   & \textbf{Opt.}                 & 56640.0                         & 759.3   & 8.87     & 8/10   & \textbf{Opt.}   & \textbf{56639.0}    & 805.4   & 11.83    \\
fl1400                    & 20127                 & 0/10   & \textbf{20164}                & \textbf{20165.5}                & 1400.0  & 1132.95  & 0/10   & \textbf{20164}  & \textbf{20165.5}    & 1400.0  & 1356.33  \\
fl1577                    & 22249                 & 0/10   & \textbf{22254}                & 22260.6                         & 1577.0  & 1172.10  & 0/10   & \textbf{22254}  & \textbf{22260.3}    & 1577.0  & 1672.84  \\
vm1748                    & 336556                & 9/10   & \textbf{Opt.}                 & 336557.3                        & 1007.9  & 12.69    & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 319.7   & 9.62     \\
u1817                     & 57201                 & 1/10   & \textbf{Opt.}                 & 57251.1                         & 1817.0  & 74.19    & 3/10   & \textbf{Opt.}   & \textbf{57233.1}    & 1643.8  & 151.69   \\
rl1889                    & 316536                & 0/10   & 316549                        & 316549.8                        & 1889.0  & 61.40    & 1/10   & \textbf{Opt.}   & \textbf{316547.7}   & 1728.7  & 77.32    \\
d2103                     & 80450                 & 0/10   & 80471                         & 80505.7                         & 2103.0  & 67.07    & 3/10   & \textbf{Opt.}   & \textbf{80479.4}    & 1707.9  & 92.11    \\
u2152                     & 64253                 & 3/10   & \textbf{Opt.}                 & 64287.7                         & 1614.0  & 73.81    & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 606.6   & 55.76    \\
pcb3038                   & 137694                & 4/10   & \textbf{Opt.}                 & 137701.2                        & 2078.6  & 69.56    & 6/10   & \textbf{Opt.}   & \textbf{137696.0}   & 1548.4  & 115.83   \\
fl3795                    & 28772                 & 4/10   & \textbf{Opt.}                 & \textbf{28783.2}                & 2998.1  & 423.94   & 3/10   & \textbf{Opt.}   & 28794.5             & 2825.1  & 613.97   \\
fnl4461                   & 182566                & 9/10   & \textbf{Opt.}                 & 182566.5                        & 923.1   & 31.05    & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 243.1   & 16.84    \\
rl5915                    & 565530                & 1/10   & \textbf{Opt.}                 & 565621.5                        & 5915.0  & 242.05   & 0/10   & 565585          & \textbf{565606.3}   & 5915.0  & 409.91   \\
rl5934                    & 556045                & 0/10   & 556172                        & 556377.6                        & 5934.0  & 305.02   & 2/10   & \textbf{Opt.}   & \textbf{556244.3}   & 5829.7  & 528.23   \\
rl11849                   & 923288                & 2/10   & \textbf{Opt.}                 & 923362.7                        & 10933.4 & 2281.04  & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 3808.7  & 1724.79  \\
usa13509                  & 19982859              & 1/10   & \textbf{Opt.}                 & 19983103.4                      & 13509.0 & 3087.15  & 4/10   & \textbf{Opt.}   & \textbf{19982999.8} & 11231.4 & 9230.64  \\
brd14051                  & 469385                & 0/10   & \textbf{469390}               & \textbf{469399.3}               & 14051.0 & 4788.59  & 0/10   & 469392          & 469405.9            & 14051.0 & 12061.60 \\
d15112                    & 1573084               & 0/10   & 1573110                       & \textbf{1573153.5}              & 15112.0 & 6587.25  & 1/10   & \textbf{Opt.}   & 1573197.3           & 14371.1 & 15462.40 \\
d18512                    & 645238                & 0/10   & \textbf{645250}               & \textbf{645263.0}               & 18512.0 & 10242.33 & 0/10   & \textbf{645250} & 645270.7            & 18512.0 & 21464.69 \\
pla33810                  & 66048945 & 0/5 & 66061689 & 66065656.2 & 3000.0  & 46448.37 & 0/5    & \textbf{66051385}               & \textbf{66055594.0}                 & 3000.0      & 83559.086 \\
pla85900                  & 142382641             & 0/5    & \multicolumn{1}{l}{142455345} & \multicolumn{1}{l}{142457070.8} & 3000.0  & 14693.79 & 0/5    & \textbf{142418516}               & \textbf{142422093.4}                 & 3000.0      & 30212.37    \\ \bottomrule
\end{tabular}}
\label{tab-main}
\end{table*}

==> table-Main2.tex <==
\begin{table*}[t]
\centering
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{lr|rrrrr|rrrrr} \toprule
\multirow{2}{*}{Instance} & \multirow{2}{*}{Opt.~~} & \multicolumn{5}{c|}{LKH}                                             & \multicolumn{5}{c}{MABB-LKH}                                         \\ \cline{3-7} \cline{8-12}
                          &                       & Success & Best            & Average            & Trials  & Time (s)  & Success & Best            & Average             & Trials  & Time (s)  \\ \hline
%ch150                     & 6528                  & 9/10   & \textbf{Opt.}   & \textbf{6528.5}    & 60.1    & 0.05     & 4/10   & \textbf{Opt.}   & 6531.0              & 115.5   & 0.05     \\
%kroB150                   & 26130                 & 2/10   & \textbf{Opt.}   & \textbf{26131.6}   & 128.4   & 0.24     & 1/10   & \textbf{Opt.}   & 26131.8             & 146.6   & 0.11     \\
%si175                     & 21407                 & 7/10   & \textbf{Opt.}   & \textbf{21407.3}   & 105.9   & 6.15     & 5/10   & \textbf{Opt.}   & 21407.5             & 136.8   & 6.64     \\
%rat195                    & 2323                  & 9/10   & \textbf{Opt.}   & \textbf{2323.5}    & 55.0    & 0.15     & 8/10   & \textbf{Opt.}   & 2324.0              & 53.0    & 0.14     \\
%gr229                     & 134602                & 2/10   & \textbf{Opt.}   & \textbf{134613.2}  & 203.1   & 0.20     & 2/10   & \textbf{Opt.}   & \textbf{134613.2}   & 194.1   & 0.14     \\
%pr299                     & 48191                 & 9/10   & \textbf{Opt.}   & 48194.3            & 51.7    & 0.36     & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 27.0    & 0.29     \\
%lin318                    & 42029                 & 4/10   & \textbf{Opt.}   & 42085.4            & 249.3   & 0.55     & 8/10   & \textbf{Opt.}   & \textbf{42051.8}    & 128.6   & 0.22     \\
%gr431                     & 171414                & 3/10   & \textbf{Opt.}   & 171499.2           & 347.0   & 1.73     & 3/10   & \textbf{Opt.}   & \textbf{171498.0}   & 370.0   & 1.73     \\
%pr439                     & 107217                & 10/10  & \textbf{Opt.}   & \textbf{Opt.}      & 39.5    & 0.50     & 9/10   & \textbf{Opt.}   & 107224.2            & 143.3   & 1.01     \\
%d493                      & 35002                 & 2/10   & \textbf{Opt.}   & \textbf{35003.6}   & 419.3   & 2.62     & 1/10   & \textbf{Opt.}   & 35003.8             & 447.5   & 2.98     \\
si535                     & 48450                 & 7/10   & \textbf{Opt.}   & 48451.1            & 311.6   & 21.28    & 8/10   & \textbf{Opt.}   & \textbf{48450.8}    & 290.3   & 15.52    \\
rat575                    & 6773                  & 2/10   & \textbf{Opt.}   & 6773.8             & 526.9   & 2.32     & 4/10   & \textbf{Opt.}   & \textbf{6773.6}     & 446.7   & 2.49     \\
gr666                     & 294358                & 5/10   & \textbf{Opt.}   & \textbf{294417.0}  & 459.8   & 2.41     & 2/10   & \textbf{Opt.}   & 294452.4            & 567.8   & 2.89     \\
pr1002                    & 259045                & 8/10   & \textbf{Opt.}   & 259045.6           & 549.0   & 3.13     & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 172.8   & 1.10     \\
u1060                     & 224094                & 5/10   & \textbf{Opt.}   & 224107.5           & 663.3   & 84.17    & 9/10   & \textbf{Opt.}   & \textbf{224096.7}   & 182.7   & 30.02    \\
vm1084                    & 239297                & 3/10   & \textbf{Opt.}   & 239372.6           & 824.1   & 32.98    & 5/10   & \textbf{Opt.}   & \textbf{239336.0}   & 767.0   & 35.48    \\
pcb1173                   & 56892                 & 4/10   & \textbf{Opt.}   & 56895.0            & 844.0   & 3.92     & 6/10   & \textbf{Opt.}   & \textbf{56894.0}    & 658.2   & 4.11     \\
d1291                     & 50801                 & 5/10   & \textbf{Opt.}   & 50840.0            & 995.4   & 27.44    & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 614.1   & 15.18    \\
rl1304                    & 252948                & 3/10   & \textbf{Opt.}   & 253156.4           & 1170.0  & 12.48    & 7/10   & \textbf{Opt.}   & \textbf{252996.4}   & 663.4   & 12.21    \\
rl1323                    & 270199                & 6/10   & \textbf{Opt.}   & 270219.6           & 718.8   & 9.63     & 8/10   & \textbf{Opt.}   & \textbf{270204.4}   & 641.7   & 8.51     \\
nrw1379                   & 56638                 & 6/10   & \textbf{Opt.}   & 56640.0            & 759.3   & 8.87     & 8/10   & \textbf{Opt.}   & \textbf{56639.0}    & 805.4   & 11.83    \\
fl1400                    & 20127                 & 0/10   & \textbf{20164}  & \textbf{20165.5}   & 1400.0  & 1132.95  & 0/10   & \textbf{20164}  & \textbf{20165.5}    & 1400.0  & 1356.33  \\
fl1577                    & 22249                 & 0/10   & \textbf{22254}  & 22260.6            & 1577.0  & 1172.10  & 0/10   & \textbf{22254}  & \textbf{22260.3}    & 1577.0  & 1672.84  \\
vm1748                    & 336556                & 9/10   & \textbf{Opt.}   & 336557.3           & 1007.9  & 12.69    & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 319.7   & 9.62     \\
u1817                     & 57201                 & 1/10   & \textbf{Opt.}   & 57251.1            & 1817.0  & 74.19    & 3/10   & \textbf{Opt.}   & \textbf{57233.1}    & 1643.8  & 151.69   \\
rl1889                    & 316536                & 0/10   & 316549          & 316549.8           & 1889.0  & 61.40    & 1/10   & \textbf{Opt.}   & \textbf{316547.7}   & 1728.7  & 77.32    \\
d2103                     & 80450                 & 0/10   & 80471           & 80505.7            & 2103.0  & 67.07    & 3/10   & \textbf{Opt.}   & \textbf{80479.4}    & 1707.9  & 92.11    \\
u2152                     & 64253                 & 3/10   & \textbf{Opt.}   & 64287.7            & 1614.0  & 73.81    & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 606.6   & 55.76    \\
pcb3038                   & 137694                & 4/10   & \textbf{Opt.}   & 137701.2           & 2078.6  & 69.56    & 6/10   & \textbf{Opt.}   & \textbf{137696.0}   & 1548.4  & 115.83   \\
fl3795                    & 28772                 & 4/10   & \textbf{Opt.}   & \textbf{28783.2}   & 2998.1  & 423.94   & 3/10   & \textbf{Opt.}   & 28794.5             & 2825.1  & 613.97   \\
fnl4461                   & 182566                & 9/10   & \textbf{Opt.}   & 182566.5           & 923.1   & 31.05    & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 243.1   & 16.84    \\
rl5915                    & 565530                & 1/10   & \textbf{Opt.}   & 565621.5           & 5915.0  & 242.05   & 0/10   & 565585          & \textbf{565606.3}   & 5915.0  & 409.91   \\
rl5934                    & 556045                & 0/10   & 556172          & 556377.6           & 5934.0  & 305.02   & 2/10   & \textbf{Opt.}   & \textbf{556244.3}   & 5829.7  & 528.23   \\
rl11849                   & 923288                & 2/10   & \textbf{Opt.}   & 923362.7           & 10933.4 & 2281.04  & 10/10  & \textbf{Opt.}   & \textbf{Opt.}       & 3808.7  & 1724.79  \\
usa13509                  & 19982859              & 1/10   & \textbf{Opt.}   & 19983103.4         & 13509.0 & 3087.15  & 4/10   & \textbf{Opt.}   & \textbf{19982999.8} & 11231.4 & 9230.64  \\
brd14051                  & 469385                & 0/10   & \textbf{469390} & \textbf{469399.3}  & 14051.0 & 4788.59  & 0/10   & 469392          & 469405.9            & 14051.0 & 12061.60 \\
d15112                    & 1573084               & 0/10   & 1573110         & \textbf{1573153.5} & 15112.0 & 6587.25  & 1/10   & \textbf{Opt.}   & 1573197.3           & 14371.1 & 15462.40 \\
d18512                    & 645238                & 0/10   & \textbf{645250} & \textbf{645263.0}  & 18512.0 & 10242.33 & 0/10   & \textbf{645250} & 645270.7            & 18512.0 & 21464.69 \\
%pla33810                  & 66048945              & 0/2    & 0               & 0.0                & 0.0     & 0.00     & 0/2    & 0               & 0.0                 & 0.0     & 0.00     \\
pla85900                  & 142382641             & 0/5    & 142455345               & 142457070.8                & 3000.0     & 14693.79     & 0/5    & 0               & 0.0                 & 3000.0     & 0.00    \\ \bottomrule
\end{tabular}}
\caption{Detailed comparisonal results of \name and LKH. The best results appear in \bf{\textbf{bold}}. }
\label{tab-main}
\end{table*}

==> table-cvrptw-solomon-100-EXACT.tex <==
\begin{table*}[!t]
\centering
\footnotesize
% \resizebox{\linewidth}{!}{

\begin{tabular}{lrrrrrrrrr} \toprule
             & \multicolumn{4}{c}{LKH-3}                                                                                         & \multicolumn{1}{c}{} & \multicolumn{4}{c}{\name-3}                                                                        \\ \cline{2-5} \cline{7-10}
100 customer & \multicolumn{1}{r}{Best} & \multicolumn{1}{r}{Average} & \multicolumn{1}{r}{Trials} & \multicolumn{1}{r}{Time(s)} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{Best} & \multicolumn{1}{r}{Average} & \multicolumn{1}{r}{Trials} & \multicolumn{1}{r}{Time(s)} \\  \hline
C1           & \textbf{828377.78}       & \textbf{828377.78}          & 342.6                      & 0.11                        &                      & \textbf{828377.78}       & \textbf{828377.78}          & 373.6                      & 0.13                        \\
C2           & \textbf{589857.50}       & \textbf{589857.50}          & 25.5                       & 0.02                        &                      & \textbf{589857.50}       & \textbf{589857.50}          & 39.3                       & 0.03                        \\
R1           & 1212747.83               & 1219946.50                  & 6794.6                     & 30.29                       &                      & \textbf{1210759.08}      & \textbf{1215941.05}         & 5801.9                     & 50.50                       \\
R2           & \textbf{952589.27}       & \textbf{957181.87}          & 7112.8                     & 45.44                       &                      & 952934.73                & 958845.88                   & 7110.9                     & 131.74                      \\
RC1          & \textbf{1364209.13}      & \textbf{1387606.83}         & 8440.8                     & 28.54                       &                      & 1379580.88               & 1394140.07                  & 7570.1                     & 45.93                       \\
RC2          & 1122912.63               & 1129167.75                  & 7315.5                     & 47.89                       &                      & \textbf{1119537.75}      & \textbf{1128636.21}         & 8332.3                     & 101.97                     \\ \bottomrule
\end{tabular}

\caption{The Comparison between \name-3 and LKH-3 in Solomon\_100\_EXACT of CVRPTW. The best results appear in \textbf{bold}.}
\label{cvrptw-solomon-100-EXACT}
\end{table*}
